Stock Price Predictability and the Business Cycle via Machine Learning

We study the impacts of business cycles on machine learning (ML) predictions. Using the S&P 500 index, we find that ML models perform worse during most recessions, and the inclusion of recession history or the risk-free rate does not necessarily improve their performance. Investigating recessions where models perform well, we find that they exhibit lower market volatility than other recessions. This implies that the improved performance is not due to the merit of ML methods but rather factors such as effective monetary policies that stabilized the market. We recommend that ML practitioners evaluate their models during both recessions and expansions.

==> tables/comparisons.tex <==
\begin{singlespace}
\begin{table}[htbp]
    \caption[Model Performance Comparisons.]{Model Performance Comparisons. Each row of the table describes the statistics calculated to answer each research question. The second column describes the research question addressed. The third column describes the performance comparisons made. E.g., For research question 1, the performance of each model on the non-recession OOS set and recession OOS set were compared and the number of models with better performances during non-recession was counted.}
    % {\bf LI RONG: this caption probably can be reduced a bit. Also, the entire table might be reduced - I think research questions are sufficiently clear as these are now highlighted in the intro, so you don't need to reproduce them word-for-word here, simplify them to save space} LR: I assume we are removing this table, so I shall just leave this as it is for now. 
    \label{tab:comparisons} 
    \centering
    \begin{tabularx}{\textwidth}{L{0.01}L{0.6}L{0.39}}
    \hline
        & \textbf{Research Questions} & \textbf{Calculate Proportion of Models with Improved OOS Performance} \\ \hline 
        1 & Do SPF models perform worse during the recession compared to non-recession? & During non-recession days compared to recession days \\ 
        2 & Does including recession data in the ISS improve SPF performance? & Before and after including recession data to ISS  \\ 
        3 & Does the risk-free rate predictor improve SPF performance? & Befor and after adding risk-free rate as a predictor \\ 
    \end{tabularx}
\end{table}
\end{singlespace}
